Hybrid Behaviour of Markov Population Models

We investigate the behaviour of population models written in Stochastic Concurrent Constraint Programming (sCCP), a stochastic extension of Concurrent Constraint Programming. In particular, we focus on models from which we can define a semantics of sCCP both in terms of Continuous Time Markov Chains (CTMC) and in terms of Stochastic Hybrid Systems, in which some populations are approximated continuously, while others are kept discrete. We will prove the correctness of the hybrid semantics from the point of view of the limiting behaviour of a sequence of models for increasing population size. More specifically, we prove that, under suitable regularity conditions, the sequence of CTMC constructed from sCCP programs for increasing population size converges to the hybrid system constructed by means of the hybrid semantics. We investigate in particular what happens for sCCP models in which some transitions are guarded by boolean predicates or in the presence of instantaneous transitions.

==> figs/csHa.tex <==

\definecolor{lb}{RGB}{168,223,221}

\begin{tikzpicture}[node distance=3cm,on grid]
  \node[state,fill = lb]  (S) {Server};
 
  \node[state,fill = lb] (C) [right =of S] {\mbox{Client $\frac{dX_r}{dt} = k_tX_t - \min\{k_r X_r,k_s X_i\}$}};
  \node[state,fill = lb] (SC) [right =of C] {$I$};

\path (S) edge [->,left,out=120,in=180] node {inf} (S)
      (S) edge [->,below,out=180,in=240] node {rec} (S) 
      (C) edge [->,right] node {susc} (S);
\end{tikzpicture}

